Luminosity determination in pp collisions at $\sqrt{s}$ = 8 TeV using the ATLAS detector at the LHC

The luminosity determination for the ATLAS detector at the LHC during pp collisions at $\sqrt{s}$ = 8 TeV in 2012 is presented. The evaluation of the luminosity scale is performed using several luminometers, and comparisons between these luminosity detectors are made to assess the accuracy, consistency and long-term stability of the results. A luminosity uncertainty of dL/L = +/- 1.9% is obtained for the 22.7 fb$^{-1}$ of pp collision data delivered to ATLAS at $\sqrt{s}$ = 8 TeV in 2012.

==> auxMat.tex <==
\appendix
\section*{Auxiliary material: delivered luminosity per LHC fill and per ATLAS run}

\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}

%% Table~\ref{tab:intLumPerFill} lists the integrated luminosity per LHC fill delivered in 2012 to the ATLAS experiment, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are excluded.

\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline	
2488 & 200967 & 07/04 22:49:28 & 08/04 03:09:30 & 10.02 \\
2489 & 200967 & 08/04 05:17:05 & 08/04 09:32:22 & 11.35 \\
2491 & 200987 & 08/04 16:20:41 & 09/04 02:37:44 & 57.13 \\
2493 & 201006 & 09/04 08:32:40 & 09/04 14:58:05 & 41.68 \\
2497 & 201052 & 10/04 02:03:34 & 10/04 04:50:24 & 21.80 \\
2500 & 201113 & 10/04 18:00:44 & 10/04 23:46:43 & 35.89 \\
2501 & 201120 & 11/04 06:00:14 & 11/04 08:47:01 & 19.14 \\
2505 & 201138 & 11/04 16:01:24 & 12/04 00:04:35 & 47.33 \\
2508 & 201190 & 12/04 14:02:49 & 12/04 20:16:35 & 49.65 \\
2509 & 201191 & 12/04 23:19:50 & 13/04 05:07:02 & 46.20 \\
2513 & 201257 & 14/04 01:12:26 & 14/04 11:43:00 & 89.28 \\
2514 & 201269 & 14/04 14:16:03 & 14/04 23:16:22 & 79.07 \\
2515 & 201280 & 15/04 09:20:17 & 15/04 10:12:15 & 11.63 \\
2516 & 201289 & 15/04 13:18:38 & 15/04 21:05:54 & 81.28 \\
2533 & 201489 & 18/04 17:52:16 & 18/04 23:54:39 & 71.02 \\
2534 & 201494 & 19/04 03:56:40 & 19/04 08:10:16 & 44.85 \\
2535 & 201555 & 19/04 16:24:07 & 19/04 19:14:46 & 38.65 \\
2536 & 201556 & 20/04 02:52:25 & 20/04 12:41:04 & 121.89 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS in April  2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. 
Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.
}
\label{tab:intLumPerF1}
\end{table}



\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline
%
2580 & 202668 & 02/05 06:06:21 & 02/05 12:53:50 & 25.34 \\
2583 & 202712 & 02/05 20:29:43 & 03/05 00:21:52 & 29.07 \\
2587 & 202798 & 03/05 18:34:32 & 04/05 01:46:20 & 51.23 \\
2590 & 202965 & 06/05 13:40:27 & 06/05 16:52:07 & 24.04 \\
2591 & 202987 & 06/05 21:55:09 & 06/05 23:14:32 & 13.68 \\
2593 & 202991 & 07/05 04:40:03 & 07/05 09:16:46 & 39.16 \\
2596 & 203027 & 07/05 20:36:28 & 08/05 07:09:18 & 87.07 \\
2609 & 203195 & 10/05 18:41:34 & 10/05 23:08:20 & 44.04 \\
2616 & 203228 & 11/05 12:04:36 & 11/05 13:59:31 & 25.03 \\
2621 & 203258 & 12/05 06:48:40 & 12/05 20:05:48 & 116.42 \\
2623 & 203277 & 13/05 02:27:20 & 13/05 07:53:01 & 59.73 \\
2624 & 203335 & 13/05 16:54:52 & 13/05 22:05:12 & 60.27 \\
2627 & 203336 & 14/05 01:28:58 & 14/05 11:36:35 & 96.83 \\
2628 & 203353 & 14/05 20:18:30 & 15/05 04:09:01 & 92.97 \\
2629 & 203432 & 15/05 12:30:37 & 15/05 18:22:17 & 67.71 \\
2630 & 203454 & 15/05 20:56:11 & 15/05 22:04:43 & 20.29 \\
2630 & 203456 & 15/05 22:23:04 & 16/05 01:09:48 & 38.60 \\
2634 & 203523 & 17/05 01:17:49 & 17/05 02:39:41 & 21.82 \\
2635 & 203524 & 17/05 04:48:41 & 17/05 10:03:05 & 75.83 \\
2644 & 203602 & 18/05 11:56:09 & 19/05 02:41:03 & 166.01 \\
2646 & 203636 & 19/05 11:15:15 & 20/05 03:20:55 & 182.73 \\
2648 & 203680 & 20/05 16:15:26 & 20/05 21:50:31 & 76.47 \\
2649 & 203719 & 21/05 11:41:39 & 21/05 19:00:49 & 106.01 \\
2651 & 203739 & 22/05 06:48:56 & 22/05 13:35:16 & 100.46 \\
2651 & 203745 & 22/05 13:51:43 & 23/05 02:24:53 & 103.09 \\
2653 & 203760 & 23/05 06:55:07 & 23/05 07:32:49 & 11.42 \\
2657 & 203779 & 23/05 16:42:25 & 23/05 22:45:09 & 89.93 \\
2658 & 203792 & 24/05 01:53:32 & 24/05 03:14:45 & 26.02 \\
2660 & 203875 & 24/05 15:35:35 & 24/05 16:49:39 & 23.65 \\
2663 & 203876 & 25/05 01:45:07 & 25/05 13:05:09 & 160.43 \\
2669 & 203934 & 26/05 04:24:25 & 26/05 12:37:49 & 128.64 \\
2670 & 204025 & 27/05 23:13:25 & 28/05 00:35:10 & 26.48 \\
2671 & 204026 & 28/05 03:34:16 & 28/05 10:50:42 & 116.13 \\
2673 & 204071 & 28/05 19:59:03 & 28/05 22:47:41 & 51.48 \\
2675 & 204073 & 29/05 04:26:34 & 29/05 08:27:32 & 74.09 \\
2683 & 204134 & 30/05 14:26:53 & 30/05 16:06:30 & 31.88 \\
2684 & 204153 & 30/05 18:33:44 & 30/05 22:01:36 & 63.63 \\
2686 & 204158 & 31/05 04:01:31 & 31/05 14:01:34 & 146.14 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS, in May 2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.
}
\label{tab:intLumPerF2}
\end{table}





\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline
%
2691 & 204240 & 01/06 11:42:04 & 02/06 01:43:50 & 163.69 \\
2692 & 204265 & 02/06 05:10:41 & 03/06 03:59:23 & 230.73 \\
2698 & 204416 & 04/06 17:26:42 & 04/06 22:28:42 & 86.83 \\
2700 & 204442 & 05/06 04:43:58 & 05/06 06:25:10 & 31.15 \\
2701 & 204474 & 05/06 09:35:11 & 05/06 21:24:56 & 153.52 \\
2710 & 204564 & 06/06 18:04:43 & 07/06 08:31:49 & 195.40 \\
2711 & 204633 & 07/06 15:04:56 & 07/06 17:45:01 & 51.22 \\
2712 & 204668 & 07/06 20:49:02 & 08/06 07:27:23 & 157.41 \\
2714 & 204726 & 08/06 16:46:11 & 08/06 18:36:43 & 36.72 \\
2717 & 204763 & 09/06 11:05:14 & 10/06 02:47:01 & 193.87 \\
2718 & 204769 & 10/06 06:51:26 & 10/06 13:22:27 & 107.72 \\
2718 & 204772 & 10/06 13:26:00 & 10/06 21:42:55 & 81.85 \\
2720 & 204796 & 11/06 02:07:50 & 11/06 02:38:51 & 10.89 \\
2723 & 204853 & 11/06 12:34:47 & 11/06 15:02:56 & 47.66 \\
2724 & 204857 & 11/06 18:03:37 & 11/06 19:17:08 & 24.92 \\
2725 & 204910 & 12/06 07:44:35 & 12/06 14:49:26 & 116.42 \\
2726 & 204932 & 12/06 20:09:06 & 13/06 05:14:29 & 138.03 \\
2728 & 204954 & 13/06 09:42:19 & 13/06 13:30:36 & 71.47 \\
2728 & 204955 & 13/06 13:49:38 & 13/06 21:35:06 & 93.27 \\
2729 & 204976 & 14/06 02:01:12 & 14/06 05:30:32 & 65.79 \\
2732 & 205010 & 14/06 18:28:39 & 14/06 20:23:20 & 39.21 \\
2733 & 205016 & 15/06 01:03:06 & 15/06 06:58:51 & 100.52 \\
2733 & 205017 & 15/06 07:11:13 & 15/06 13:56:32 & 71.85 \\
2734 & 205055 & 15/06 20:51:07 & 16/06 12:24:53 & 198.39 \\
2736 & 205071 & 16/06 18:10:32 & 17/06 11:40:57 & 228.91 \\
2737 & 205112 & 17/06 18:58:41 & 17/06 22:39:04 & 64.54 \\
2739 & 205113 & 18/06 08:30:02 & 18/06 11:02:15 & 49.67 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS, in June 2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.}
\label{tab:intLumPerF3}
\end{table}


\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline
%
2805 & 206368 & 03/07 20:09:45 & 04/07 04:07:13 & 57.92 \\
2806 & 206369 & 04/07 07:31:55 & 04/07 16:49:12 & 100.11 \\
2807 & 206409 & 04/07 22:09:42 & 05/07 08:55:43 & 143.63 \\
2816 & 206564 & 07/07 15:38:00 & 07/07 21:45:16 & 93.67 \\
2816 & 206573 & 08/07 00:21:36 & 08/07 03:29:03 & 28.40 \\
2819 & 206614 & 08/07 17:39:26 & 08/07 18:48:17 & 20.91 \\
2840 & 206955 & 13/07 21:24:39 & 13/07 22:41:14 & 22.58 \\
2842 & 206962 & 14/07 04:58:58 & 14/07 16:31:06 & 144.14 \\
2843 & 206971 & 14/07 19:18:17 & 15/07 03:13:40 & 110.81 \\
2847 & 207044 & 15/07 15:45:10 & 15/07 19:43:27 & 64.28 \\
2848 & 207046 & 15/07 22:19:15 & 16/07 07:42:02 & 124.82 \\
2858 & 207221 & 20/07 04:44:50 & 20/07 18:21:30 & 170.36 \\
2861 & 207262 & 21/07 01:39:35 & 21/07 02:37:36 & 19.02 \\
2870 & 207304 & 21/07 22:32:58 & 22/07 06:58:21 & 108.50 \\
2871 & 207306 & 22/07 09:49:25 & 22/07 14:46:15 & 74.47 \\
2872 & 207332 & 22/07 17:05:30 & 23/07 08:10:42 & 162.08 \\
2873 & 207397 & 23/07 20:15:25 & 24/07 08:15:20 & 147.96 \\
2875 & 207447 & 24/07 15:46:06 & 25/07 07:10:45 & 168.13 \\
2880 & 207490 & 26/07 02:08:19 & 26/07 11:26:12 & 114.51 \\
2884 & 207531 & 27/07 02:31:55 & 27/07 04:47:23 & 37.02 \\
2884 & 207532 & 27/07 04:51:53 & 27/07 12:12:34 & 79.65 \\
2886 & 207582 & 27/07 21:10:13 & 28/07 00:54:24 & 59.41 \\
2887 & 207589 & 28/07 03:22:20 & 28/07 08:09:50 & 74.41 \\
2888 & 207620 & 28/07 14:42:35 & 29/07 06:31:23 & 178.13 \\
2891 & 207664 & 29/07 16:05:23 & 29/07 22:15:17 & 95.20 \\
2892 & 207696 & 30/07 02:26:40 & 30/07 12:28:31 & 134.74 \\
2893 & 207749 & 30/07 21:22:54 & 31/07 02:02:17 & 73.67 \\
2894 & 207772 & 31/07 04:41:22 & 31/07 05:38:44 & 17.84 \\
2898 & 207809 & 31/07 17:21:20 & 01/08 06:43:54 & 159.43 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS, in July 2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.}
\label{tab:intLumPerF4}
\end{table}





\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline
%
2900 & 207845 & 01/08 13:59:20 & 01/08 17:28:34 & 58.52 \\
2902 & 207864 & 01/08 21:33:27 & 01/08 23:42:54 & 39.88 \\
2902 & 207865 & 02/08 01:47:41 & 02/08 10:09:45 & 86.29 \\
2906 & 207931 & 03/08 01:43:44 & 03/08 02:39:52 & 17.81 \\
2908 & 207934 & 03/08 07:18:15 & 03/08 17:15:05 & 131.61 \\
2911 & 207975 & 04/08 06:00:08 & 04/08 10:47:43 & 59.91 \\
2912 & 207982 & 04/08 13:29:00 & 04/08 21:14:34 & 117.91 \\
2918 & 208123 & 06/08 17:08:42 & 06/08 22:25:27 & 68.67 \\
2920 & 208126 & 07/08 03:05:55 & 07/08 04:22:46 & 25.76 \\
2927 & 208184 & 07/08 23:30:18 & 08/08 07:32:38 & 102.75 \\
2928 & 208189 & 08/08 10:11:15 & 08/08 12:34:51 & 44.05 \\
2929 & 208258 & 08/08 18:04:18 & 08/08 23:48:27 & 90.53 \\
2932 & 208261 & 09/08 03:35:14 & 09/08 10:01:48 & 100.13 \\
2934 & 208354 & 09/08 21:26:09 & 10/08 06:23:11 & 129.89 \\
2957 & 208485 & 12/08 22:31:28 & 13/08 07:55:39 & 138.83 \\
2976 & 208662 & 15/08 17:47:53 & 16/08 05:07:42 & 145.42 \\
2978 & 208705 & 16/08 13:07:22 & 16/08 14:24:32 & 26.88 \\
2980 & 208717 & 16/08 22:22:58 & 17/08 01:10:49 & 54.51 \\
2981 & 208720 & 17/08 04:00:55 & 17/08 05:01:09 & 22.48 \\
2983 & 208780 & 17/08 13:41:45 & 17/08 15:47:42 & 44.15 \\
2983 & 208781 & 17/08 16:16:58 & 18/08 05:37:09 & 143.51 \\
2984 & 208811 & 18/08 08:04:32 & 19/08 03:15:26 & 218.37 \\
2987 & 208870 & 19/08 11:23:19 & 19/08 12:01:32 & 14.27 \\
2991 & 208930 & 20/08 16:36:24 & 20/08 19:56:23 & 63.03 \\
2991 & 208931 & 20/08 20:09:56 & 21/08 06:20:54 & 105.06 \\
2992 & 208970 & 21/08 14:11:19 & 21/08 20:52:35 & 103.07 \\
2993 & 208982 & 22/08 03:47:25 & 22/08 15:53:30 & 175.38 \\
2996 & 209074 & 23/08 14:31:09 & 23/08 18:11:57 & 69.44 \\
2997 & 209084 & 23/08 20:45:46 & 24/08 02:00:46 & 97.74 \\
2998 & 209109 & 24/08 06:30:59 & 24/08 14:03:18 & 131.69 \\
3000 & 209161 & 24/08 21:36:50 & 25/08 00:01:22 & 51.27 \\
3002 & 209183 & 25/08 07:33:41 & 25/08 20:16:21 & 173.31 \\
3003 & 209214 & 25/08 23:49:27 & 26/08 00:32:00 & 16.64 \\
3005 & 209254 & 26/08 07:04:47 & 26/08 15:24:15 & 129.28 \\
3007 & 209269 & 26/08 22:54:23 & 27/08 01:41:33 & 56.93 \\
3011 & 209381 & 28/08 00:10:08 & 28/08 12:11:15 & 172.58 \\
3016 & 209550 & 30/08 22:03:29 & 31/08 07:00:42 & 124.63 \\
3018 & 209580 & 31/08 16:55:22 & 01/09 06:04:57 & 168.67 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS, in August 2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.}
\label{tab:intLumPerF5}
\end{table}





\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline
%
3019 & 209608 & 01/09 09:35:51 & 01/09 15:12:23 & 89.75 \\
3020 & 209628 & 01/09 23:24:08 & 02/09 04:18:06 & 85.36 \\
3021 & 209629 & 02/09 07:09:32 & 02/09 20:06:47 & 163.96 \\
3025 & 209736 & 03/09 18:29:36 & 04/09 04:08:45 & 130.28 \\
3027 & 209776 & 04/09 12:19:50 & 04/09 13:36:39 & 24.54 \\
3029 & 209787 & 04/09 21:49:52 & 05/09 04:35:33 & 116.99 \\
3032 & 209812 & 05/09 13:58:27 & 05/09 16:05:06 & 38.86 \\
3032 & 209812 & 05/09 16:18:19 & 05/09 23:09:35 & 79.89 \\
3033 & 209864 & 06/09 09:13:07 & 06/09 18:53:09 & 142.44 \\
3034 & 209866 & 06/09 21:29:29 & 06/09 22:54:56 & 33.05 \\
3036 & 209899 & 07/09 04:00:35 & 07/09 09:35:06 & 100.21 \\
3039 & 209909 & 07/09 21:52:54 & 07/09 22:41:09 & 18.84 \\
3045 & 209980 & 08/09 20:22:13 & 09/09 08:35:02 & 172.96 \\
3047 & 209995 & 09/09 17:56:07 & 10/09 04:04:10 & 133.32 \\
3067 & 210302 & 15/09 17:48:36 & 16/09 07:30:56 & 162.76 \\
3071 & 210308 & 16/09 18:08:37 & 17/09 04:05:15 & 139.27 \\
3108 & 211620 & 28/09 06:01:48 & 28/09 07:42:47 & 17.52 \\
3109 & 211670 & 28/09 16:41:04 & 28/09 19:27:15 & 24.81 \\
3110 & 211697 & 29/09 04:30:28 & 29/09 05:11:25 & 11.95 \\
3113 & 211772 & 30/09 03:22:18 & 30/09 11:25:48 & 101.43 \\
3114 & 211787 & 30/09 14:23:46 & 01/10 01:12:49 & 146.72 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS, in September 2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.}
\label{tab:intLumPerF6}
\end{table}





\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline
%
3121 & 211867 & 01/10 22:38:32 & 02/10 10:31:08 & 148.37 \\
3124 & 211902 & 02/10 20:28:49 & 02/10 21:24:11 & 18.49 \\
3126 & 211937 & 03/10 03:51:46 & 03/10 10:13:42 & 110.75 \\
3129 & 212034 & 04/10 01:49:05 & 04/10 06:26:22 & 81.56 \\
3131 & 212142 & 05/10 00:51:57 & 05/10 04:21:43 & 66.32 \\
3133 & 212144 & 05/10 10:17:55 & 06/10 00:48:42 & 183.96 \\
3134 & 212172 & 06/10 03:39:18 & 06/10 16:07:55 & 174.77 \\
3135 & 212199 & 06/10 18:29:46 & 07/10 04:32:15 & 155.04 \\
3138 & 212272 & 07/10 15:04:06 & 08/10 01:00:05 & 146.80 \\
3178 & 212663 & 14/10 05:49:46 & 14/10 08:11:11 & 47.40 \\
3182 & 212687 & 14/10 20:58:44 & 15/10 01:16:40 & 75.91 \\
3185 & 212721 & 15/10 10:43:23 & 15/10 18:31:33 & 119.89 \\
3188 & 212742 & 16/10 02:03:10 & 16/10 09:01:01 & 103.67 \\
3191 & 212809 & 16/10 21:57:55 & 16/10 22:45:41 & 15.97 \\
3192 & 212815 & 17/10 01:22:11 & 17/10 13:00:17 & 151.13 \\
3194 & 212858 & 17/10 17:42:00 & 18/10 06:18:18 & 162.13 \\
3200 & 212967 & 19/10 09:10:53 & 19/10 17:29:38 & 103.23 \\
3201 & 212993 & 19/10 23:01:02 & 20/10 09:19:18 & 130.69 \\
3203 & 213039 & 20/10 18:21:14 & 21/10 06:05:35 & 170.25 \\
3204 & 213079 & 21/10 09:25:54 & 21/10 17:41:46 & 108.32 \\
3207 & 213092 & 21/10 23:58:07 & 22/10 04:17:43 & 86.75 \\
3208 & 213130 & 22/10 11:31:22 & 22/10 15:44:40 & 74.83 \\
3209 & 213155 & 22/10 23:22:55 & 23/10 02:03:08 & 52.62 \\
3210 & 213157 & 23/10 04:36:15 & 23/10 07:47:17 & 65.12 \\
3212 & 213204 & 23/10 16:23:29 & 23/10 17:21:25 & 21.19 \\
3214 & 213250 & 24/10 01:41:35 & 24/10 07:08:24 & 94.41 \\
3223 & 213314 & 25/10 20:53:42 & 25/10 22:27:38 & 33.45 \\
3226 & 213359 & 26/10 07:19:11 & 26/10 09:06:20 & 37.83 \\
3229 & 213431 & 27/10 01:37:53 & 27/10 06:00:18 & 86.13 \\
3231 & 213480 & 27/10 13:51:14 & 27/10 14:29:43 & 12.89 \\
3232 & 213486 & 27/10 16:51:14 & 28/10 03:32:09 & 157.54 \\
3236 & 213539 & 28/10 17:09:10 & 29/10 11:09:57 & 212.88 \\
3238 & 213627 & 29/10 21:56:50 & 29/10 23:22:25 & 30.00 \\
3238 & 213640 & 29/10 23:31:30 & 30/10 02:36:05 & 49.07 \\
3240 & 213684 & 30/10 11:40:10 & 30/10 13:07:51 & 32.08 \\
3242 & 213695 & 30/10 18:38:12 & 30/10 23:07:38 & 83.27 \\
3244 & 213702 & 31/10 03:13:44 & 31/10 05:28:19 & 48.99 \\
3249 & 213754 & 31/10 20:43:18 & 01/11 11:43:45 & 195.00 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS, in October 2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.}
\label{tab:intLumPerF7}
\end{table}





\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} % Column formatting, @{} suppresses leading/trailing space
\hline
LHC 			& ATLAS 		& From			& To					& Integrated luminosity 	\\	
 fill number	& run number	& (start time, UTC)	& (end time, UTC)		& [$\mathrm{pb}^{-1}$] 	\\
\hline
%
3250 & 213796 & 01/11 14:57:06 & 01/11 19:13:18 & 82.51 \\
3252 & 213816 & 02/11 01:48:01 & 02/11 05:01:02 & 64.60 \\
3253 & 213819 & 02/11 07:46:21 & 02/11 11:40:40 & 78.17 \\
3259 & 213900 & 02/11 22:39:49 & 03/11 08:06:44 & 141.27 \\
3261 & 213951 & 03/11 18:14:58 & 03/11 23:57:19 & 104.04 \\
3262 & 213964 & 04/11 03:00:23 & 04/11 03:31:22 & 10.43 \\
3264 & 213968 & 04/11 11:54:09 & 04/11 13:28:16 & 32.94 \\
3265 & 214021 & 05/11 00:32:14 & 05/11 14:09:56 & 180.84 \\
3266 & 214086 & 05/11 21:17:17 & 06/11 13:28:56 & 195.58 \\
3269 & 214160 & 07/11 12:43:10 & 08/11 01:11:48 & 185.02 \\
3272 & 214176 & 08/11 12:33:06 & 08/11 16:01:00 & 68.80 \\
3273 & 214216 & 09/11 01:48:48 & 09/11 09:47:43 & 123.66 \\
3279 & 214388 & 11/11 19:51:40 & 11/11 20:59:52 & 23.74 \\
3279 & 214390 & 11/11 21:12:37 & 12/11 03:37:15 & 90.66 \\
3285 & 214494 & 13/11 12:56:55 & 13/11 23:08:50 & 151.45 \\
3286 & 214523 & 14/11 02:31:47 & 14/11 12:55:07 & 158.65 \\
3287 & 214544 & 14/11 18:32:12 & 15/11 03:33:46 & 135.05 \\
3288 & 214553 & 15/11 05:58:03 & 15/11 19:03:14 & 173.72 \\
3292 & 214618 & 16/11 04:16:53 & 16/11 07:57:43 & 67.21 \\
3293 & 214651 & 16/11 10:27:29 & 16/11 11:45:44 & 28.00 \\
3296 & 214680 & 17/11 07:23:51 & 17/11 19:51:05 & 174.65 \\
3298 & 214721 & 18/11 01:28:46 & 18/11 04:45:07 & 67.63 \\
3299 & 214758 & 18/11 09:53:51 & 18/11 21:39:03 & 170.25 \\
3300 & 214777 & 19/11 04:38:38 & 19/11 13:06:13 & 143.45 \\
3318 & 215027 & 24/11 08:52:03 & 24/11 19:24:00 & 139.91 \\
3319 & 215061 & 24/11 22:31:32 & 25/11 00:50:17 & 42.11 \\
3322 & 215063 & 25/11 03:53:47 & 25/11 15:08:39 & 159.65 \\
3323 & 215091 & 25/11 18:21:34 & 26/11 05:04:14 & 158.12 \\
3347 & 215414 & 30/11 01:17:39 & 30/11 11:14:30 & 150.20 \\
3350 & 215433 & 30/11 18:10:36 & 01/12 01:57:58 & 118.62 \\
3351 & 215456 & 01/12 07:13:05 & 01/12 15:03:43 & 119.45 \\
3360 & 215464 & 02/12 02:56:14 & 02/12 15:07:39 & 167.46 \\
3363 & 215473 & 02/12 22:27:50 & 03/12 10:05:31 & 163.37 \\
3370 & 215541 & 04/12 04:29:33 & 04/12 08:32:57 & 74.94 \\
3374 & 215571 & 04/12 17:43:36 & 04/12 21:27:52 & 68.54 \\
3375 & 215589 & 05/12 05:59:22 & 05/12 09:41:23 & 70.10 \\
3378 & 215643 & 05/12 21:59:53 & 06/12 00:31:30 & 53.59 \\
\hline
 \end{tabular}
\caption{
Luminosity delivered to ATLAS, in November and December 2012, during physics data-taking in \pp\ collisions at $\sqrt s =$~8~\textrm{Te\kern -0.1em V}, per LHC fill and per ATLAS run, integrated over the intervals defined by the time stamps in the third and fourth columns. A single LHC fill can span more than one ATLAS run, and vice-versa. Commissioning fills, machine-development periods and special low-luminosity runs such as \vdM-calibration sessions are not listed.
}
\label{tab:intLumPerF8}
\end{table}



